FrankMocap: Fast Monocular 3D Hand and Body Motion Capture by Regression and Integration

Although the essential nuance of human motion is often conveyed as a combination of body movements and hand gestures, the existing monocular motion capture approaches mostly focus on either body motion capture only ignoring hand parts or hand motion capture only without considering body motion. In this paper, we present FrankMocap, a motion capture system that can estimate both 3D hand and body motion from in-the-wild monocular inputs with faster speed (9.5 fps) and better accuracy than previous work. Our method works in near real-time (9.5 fps) and produces 3D body and hand motion capture outputs as a unified parametric model structure. Our method aims to capture 3D body and hand motion simultaneously from challenging in-the-wild monocular videos. To construct FrankMocap, we build the state-of-the-art monocular 3D "hand" motion capture method by taking the hand part of the whole body parametric model (SMPL-X). Our 3D hand motion capture output can be efficiently integrated to monocular body motion capture output, producing whole body motion results in a unified parrametric model structure. We demonstrate the state-of-the-art performance of our hand motion capture system in public benchmarks, and show the high quality of our whole body motion capture result in various challenging real-world scenes, including a live demo scenario.

==> texts/overview.tex <==
\section{Tracking Overview}
\label{sec:SystemSetup}

\begin{figure}
    \centering
    % \includegraphics[width=\linewidth]{figures/temp_mugsy_hand.png}
    \includegraphics[width=\linewidth]{hand_tracking_paper/figures/Mugsy_setup.pdf}
    \caption{Example input data to our tracking method. Left: select images from the 140 cameras in our hand capture system, and right: a 3D reconstruction mesh computed with PatchMatch multi-view stereo~\cite{Galliani_2015_ICCV}. }
    % \breannan{Can we include stats on the capture system setup here?}}
    \label{fig:MugsyHand}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{hand_tracking_paper/figures/Flowchart_no-checker.pdf}
    % \includegraphics[width=\linewidth]{hand_tracking_paper/figures/Flowchart_checker.pdf}
    \caption{Overview of our dense hand surface tracking method. (a) An input image, (b) the first initialization stage using LBS, (c) the second initialization stage using a region-based deformation model, and (d) the final optimization with our combined vision and physics terms.}
    \label{fig:Flowchart}
\end{figure}

% \breannan{Should we provide a graphical flow-chart of the algorithm here?}\takaaki{Agree. Maybe something like image and/or scan mesh, LBS mesh, patch-based mesh and final mesh from left to right? }\jkh{yes, agree also.   One caution here since the early steps are building on prior work is to make sure that you spend the most time on the new contributions and not on the older work.   Otherwise the reader will conclude that the new contributions are not sufficient.}

% \breannan{We should reference the detailed sections in each paragraph, here.}\takaaki{agree}\jkh{yup}

In this section, we briefly outline our hand surface tracking algorithm before discussing each component in depth in Section~\ref{sec:Method}. 

\paragraph{Data Capture}
We first capture a hand in motion using our multi-view camera system that consists of 140 calibrated cameras with hardware synchronization, capable of capturing RGB images at 30 frames per second.
A hand is captured at the center of the cameras and lit uniformly from static LED light sources. 
% Intrinsic and extrinsic calibration parameters of the cameras are estimated using a 3D calibration target~\cite{Ha:2017:Deltille}.
% Once the cameras are calibrated, we perform the PatchMatch-based multi-view stereo algorithm~\cite{Galliani_2015_ICCV} to obtain 3D scan mesh at every frame. 
After capturing images, we perform PatchMatch-based multi-view stereo~\cite{Galliani_2015_ICCV} to obtain a 3D scan mesh for every frame. 
The images and scan mesh serve as input data of the tracking algorithm.
Figures~\ref{fig:MugsyHand} and~\ref{fig:Flowchart}(a) shows example images from our capture system and a scan mesh.
These data will be processed sequentially (\ie, starting from the beginning to the end of a sequence).


\paragraph{Hand Representation}
Similar to existing works on 3D tracking, we track a hand in motion using a template mesh.
In our setting, the template mesh is a generic surface triangle mesh designed by an artist.
From the surface mesh, we automatically compute a volumetric tetrahedral mesh on which we define a deformation energy and a collision response term.
%% Takaaki: not sure if we need to say the following...
% We choose to use these two representation together during the tracking optimization, instead of using only the tetrahedral mesh, because of flexibility for computational resource.

For every subject, we capture both the neutral pose of the hand as well as multiple motion sequences.
Given a 3D scan of the neutral pose, we manually register the template surface to the scan using the commercial ZBrush\footnote{https://pixologic.com/} modeling package, producing a personalized surface mesh. 
After registering the surface mesh, we create a volumetric tetrahedral mesh by feeding the personalized surface mesh to the TetGen library~\cite{Si:2015:TetGen}. 
Given the surface and tetrahedral meshes, we make correspondences for the surface vertices and use them in the tracking optimization.
%\breannan{Mention that/how we get exact correspondence in this step.}

% To be able to apply physics prior, we compute a tetrahedral mesh from the surface mesh by \cite{}

% We choose to have separate representations of surface mesh and tetrahedral mesh in the tracking algorithm, mainly due to the computational cost. 
% While We often use a high-resolution surface mesh for high-fidelity, tetrahedral mesh with dense surface often causes significant 
% memory consumption.
% Using the two representations and coupling them together during the optimization mitigates these issues by adjusting the density of the tetrahedral mesh surface and enables reasonable runtime cost of the optimization.





% The input to our tracking method is a sequence of multi-view images from calibrated cameras.
% We run PatchMatch-based 3D reconstruction algorithm~\cite{Galliani_2015_ICCV} to obtain 3D scan mesh at every frame.

% We capture a hand in motion with our 4D capture system that consists of 140 hardware-synchronized RGB cameras capturing images at 30 frames per second.
% A hand is captured at the center of the cameras and lit uniformly from static LED light sources. 
% Intrinsic and extrinsic calibration parameters of the cameras are estimated using a 3D calibration target~\cite{Ha:2017:Deltille}.
% Once the cameras are calibrated, we perform the PatchMatch-based multi-view stereo algorithm~\cite{Galliani_2015_ICCV} to obtain 3D scan mesh at every frame. 
% The images and scan mesh serve as input data of the tracking algorithm.
% \Fref{fig:MugsyHand} shows example images from our capture system.


% \paragraph{Data Capture} We capture a hand in motion with our 4D capture system that consists of 140 hardware-synchronized RGB cameras capturing images at 30 frames per second.
% A hand is captured at the center of the cameras and lit uniformly from static LED light sources. 
% Intrinsic and extrinsic calibration parameters of the cameras are estimated using a 3D calibration target~\cite{Ha:2017:Deltille}.
% Once the cameras are calibrated, we perform the PatchMatch-based multi-view stereo algorithm~\cite{Galliani_2015_ICCV} to obtain 3D scan mesh at every frame. 
% The images and scan mesh serve as input data of the tracking algorithm.
% \Fref{fig:MugsyHand} shows example images from our capture system.


\paragraph{Tracking Initialization}

With personalized surface and tetrahedral meshes in hand, given a sequence of images and 3D scans, we next initialize the template meshes for these sequences using a two-stage, model-based tracking optimization.
In the first stage, we deform the template using an LBS model that applies a skeleton-based transformation to local regions of the hand mesh. The embedded skeleton and skinning weights are defined by an artist before tracking and is personalized based on non-rigid registration to several frames in the beginning of the input sequence.
This step minimizes a geometric error based on the input 3D scan and the landmark error in a similar fashion to Taylor~\etal's method~\shortcite{Taylor:2016:HandTracking} (Figure~\ref{fig:Flowchart}(b)).
% \breannan{We should probably describe where joint angles and such come from here.}
% Note that this skeletal rig representation is used only during the first stage of the initialization.

In the second stage, we use a region-based linear deformation model~\cite{Tena:2011:RegionBased,Wu:2016:PatchBasedModel} to further match the template mesh to the image and 3D scan data by optimizing deformation parameters and the rigid transformations estimated in the first stage.

With the surface initialization complete, we warp the tetrahedral mesh so its surface exactly corresponds to the initialized, personalized surface triangle mesh (Figure~\ref{fig:Flowchart}(c)).
Section~\ref{ssec:InitialTracking} describes the initialization step in detail.
% Specifically, we extend a region-based linear model~\cite{Tena:2011:RegionBased,Wu:2016:PatchBasedModel} to
% a hand, where each region is parameterized with 6

% \takaaki{git test again! test2 test2}

% Two-stage initialization: LBS-based tracking, and patch model-based tracking

% \paragraph{LBS-based Tracking}

% similar to the method by Tayor and colleagues~\shortcite{Taylor:2016:HandTracking}

% LBS as the first initialization of tracking.
% Artist surface mesh with LBS. 
% Do LBS model fitting based on depth and keypoints.
% keypoint detector based on hourglass detector + multiview bootstrapping.


% \paragraph{Model-based Tracking with Region-based Model}

% Inspired by Wu and colleagues' work, we also build a patch-based model and
% get better initialization for the final tracking optimization.

% \takaaki{might need to replace ``physics prior'' below}
\paragraph{Constraining Tracking with an Elastic Physical Model}

After initializing the template, we track across a sequence by solving an optimization at each frame that includes vision-based energies, a deformable elastic energy, and an energy to couple the two representations.
This optimization alternates between refinements of surface vertex positions using the input data and updates of all tetrahedral vertex positions using the physics term until convergence.
The former optimization ensures pixel-accurate locations for visible vertices of the template mesh, while the latter optimizations deforms invisible vertices in a physically feasible manner while resolving self collisions (Figure~\ref{fig:Flowchart}(d)).
The optimization is structured in a manner that ensures a decrease in total combined energy across each alternating iteration. 
Section~\ref{sec:surftrack} describes the details of the energies and optimization.

% 4096 by 2668 pixel resolution RGB images at 30 frames per second and an exposure time of 4ms, surrounding an object at the center lit uniformly from static LED light sources. An example camera arrangement is shown in Fig.~\ref{fig:camarray}. Intrinsic and extrinsic calibration parameters for each of the cameras are computed using a planar checkerboard pattern~\cite{Zhang_TPAMI2000}.

%To our purpose, we require a stereo method not only with high accuracy but also high efficiency and scalability.
%Galliani and colleagues~\shortcite{galliani_ICCV2015} introduced a multiview PatchMatch stereo method that simultaneously propagates good random search solutions to neighbor pixels with GPUs.
% depth estimation from the 40 cameras using multiview stereo techniques. In particular, we employ the PatchMatch-based multiview stereo algorithm proposed by Galliani et al.~\cite{galliani_ICCV2015}. Our modifications are two-fold. The first is an implementation in scale-space to improve convergence. The second is a novel depth refinement scheme based on maximizing the photometric consistency. Both modifications are detailed next.



% We captur

% \paragraph{System}multiview camera system, ~140 views, 30 fps, 4K resolution

% \paragraph{Preprocessing} 3D reconstruction, LBS based on depth and keypoints

